AHAM: Adapt, Help, Ask, Model -- Harvesting LLMs for literature mining

In an era marked by a rapid increase in scientific publications, researchers grapple with the challenge of keeping pace with field-specific advances. We present the `AHAM' methodology and a metric that guides the domain-specific \textbf{adapt}ation of the BERTopic topic modeling framework to improve scientific text analysis. By utilizing the LLaMa2 generative language model, we generate topic definitions via one-shot learning by crafting prompts with the \textbf{help} of domain experts to guide the LLM for literature mining by \textbf{asking} it to model the topic names. For inter-topic similarity evaluation, we leverage metrics from language generation and translation processes to assess lexical and semantic similarity of the generated topics. Our system aims to reduce both the ratio of outlier topics to the total number of topics and the similarity between topic definitions. The methodology has been assessed on a newly gathered corpus of scientific papers on literature-based discovery. Through rigorous evaluation by domain experts, AHAM has been validated as effective in uncovering intriguing and novel insights within broad research areas. We explore the impact of domain adaptation of sentence-transformers for the task of topic \textbf{model}ing using two datasets, each specialized to specific scientific domains within arXiv and medarxiv. We evaluate the impact of data size, the niche of adaptation, and the importance of domain adaptation. Our results suggest a strong interaction between domain adaptation and topic modeling precision in terms of outliers and topic definitions.

==> text_mining_intro.tex <==

\begin{comment}
    
Text mining is a research area that deals with the construction of models and the discovery of patterns from text resources, aiming at solving tasks such as text categorization, clustering, topic identification, taxonomy construction, or sentiment analysis, to name a few~\cite{feldman2006text}. This research area, also known as text data mining or text analytics, is a multidisciplinary field drawing its techniques from data mining, machine learning, information retrieval, information extraction and natural language processing.

The standard vector representation of text units is referred to as the Bag of Words (BoW) vector representation. The BoW representation of a given text unit (a word, sentence, paragraph, or document) results in a numeric vector. In addition to BoW vector representations of text units, referred to as \emph{sparse} vector representations, different \emph{dense} text representation can be used to represent texts. Dense vector representations are usually referred to as \emph{embeddings}. The embedding technology is a prominent side effect of the advances in neural networks, where weights that can be extracted from neural networks can be used as a spatial representation that transforms relations between observed entities (data instances) into distances. Embeddings-based representations used with deep neural networks, have led to major breakthroughs in analyzing text, images, speech, and graphs~\cite{goodfellow2016deep}.

Text embeddings use large corpora of documents to extract vector representations for words, sentences, and documents. The first neural word embeddings like word2vec~\cite{mikolov2013distributed} produced one vector for each word, irrespective of its polysemy. %More recent developments like Embeddings from Language Models (ELMo)~\cite{peters2018deep} and Bidirectional Encoder Representations from Transformers (BERT)~\cite{devlin2019bert} take the context of a sentence into account and produce different word vectors for different contexts of each word.

%The most recent developments in text analysis are Large Language Models (LLMs) learned from huge text corpora. \hla{TODO Boshko}.


\end{comment}
